Complexity and Approximation Algorithms for Fixed Charge Transportation Problems

The Fixed Charge Transportation (FCT) problem models transportation scenarios where we need to send a commodity from $n$ sources to $m$ sinks, and the cost of sending a commodity from a source to a sink consists of a linear component and a fixed component. Despite extensive research on exponential time exact algorithms and heuristic algorithms for FCT and its variants, their approximability and computational complexity are not well understood. In this work, we initiate a systematic study of the approximability and complexity of these problems. When there are no linear costs, we call the problem the Pure Fixed Charge Transportation (PFCT) problem. We also distinguish between cases with general, sink-independent, and uniform fixed costs; we use the suffixes ``-S'' and ``-U'' to denote the latter two cases, respectively. This gives us six variants of the FCT problem. We give a complete characterization of the existence of $O(1)$-approximation algorithms for these variants. In particular, we give $2$-approximation algorithms for FCT-U and PFCT-S, and a $(6/5 + \epsilon)$-approximation for PFCT-U. On the negative side, we prove that FCT and PFCT are NP-hard to approximate within a factor of $O(\log^{2-\epsilon} (\max\{n, m\}))$ for any constant $\epsilon > 0$, FCT-S is NP-hard to approximate within a factor of $c\log (\max\{n, m\})$ for some constant $c> 0$, and PFCT-U is APX-hard. Additionally, we design an Efficient Parameterized Approximation Scheme (EPAS) for PFCT when parameterized by the number $n$ of sources, and an $O(1/\epsilon)$-bicriteria approximation for the FCT problem, when we are allowed to violate the demand constraints for sinks by a factor of $1\pm \epsilon$.

==> _quasi.tex <==
\newcommand{\bfT}{{\mathbf{T}}}
\newcommand{\bfr}{{\mathbf{r}}}
\newcommand{\tw}{{\mathrm{tw}}}
\newcommand{\bfE}{{\mathbf{E}}}
\newcommand{\bfV}{{\mathbf{V}}}
\newcommand{\db}{{\mathrm{db}}}

\section{Quasi-Polynomial Time Algorithm}


\label{sec:reduction}

In this section we prove Theorem~\ref{xx}, by reducing the PFCT problem to the tree labeling problem. Recall the input of the problem contains a graph $G = (V, E)$ with edge costs $c \in R_{\geq 0}^E$, a root $r$,  $k$ groups $S_1, S_2, \cdots, S_k$ of vertices, and a degree bound $\db_v \in \Z_{>0}$ for every $v \in V$.   
Without loss of generality, we assume $\{r\}, S_1, S_2, \cdots, S_k$ are mutually disjoint. Again, we use $\opt$ to denote the minimum-cost of a valid subgraph $H$.

\subsection{Preprocessing of Instance}
We process the input graph $G$ so that 
\begin{itemize}
    \item every $v \in S$ has $d_\rmin(v) = 0$ and $d_\rmout(v) = 1$,
    \item every $v \in T$ has $d_\rmin(v) = 1$ and $d_\rmout(v) = 0$, and
    \item every vertex $v$ in $V \setminus (S \cup T)$ has degree $3$, either with 2 incoming edges and 1 outgoing edge, or with 1 incoming edge or 2 outgoing edges. 
\end{itemize}
%TODO: notation?

This can be done as follows. For a source $v \in S$, we can replace $v$ with a new source $v'$, and add an edge $(v', v)$ of cost $0$ to $G$. So, the first property can be satisfied. Similarly, we can satisfy the second property.

It remains to focus on a vertex $v \in V \setminus (S \cup T)$; we can assume $d_{\rmin}(v) \geq 1$ and $d_{\rmout}(v) \geq 1$. If $d_{\rmin}(v) = d_{\rmout}(v) = 1$, then we can remove it by directly connecting its in-neighbor to its out-neighbor.  If $v$ has $d_{\rmin}(v) \geq 2$ and $d_{\rmout}(v) \geq 2$, then we can split $v$ into $v'$ and $v''$, with an edge $(v', v'')$ of $0$ cost connecting them. All the incoming edges of $v$ no go to $v'$ and all the outgoing edges of $v$ are from $v''$.  After this transformation, every vertex in $V \setminus (S \cup T)$ now has either $d_\rmin(v) = 1$ or $d_\rmout(v) = 1$.  If a vertex $v$ has $d_\rmin(v) = 1$ and $d_\rmout(v) \geq 3$, we can then replace $v$ and its incident edges with an out-arborescence, where every vertex has incoming degree 1 and outgoing degree 2. Similarly we can handle vertices $v$ with $d_\rmout(v) = 1$ and $d_\rmin(v) \geq 3$.


\subsection{Decomposition of the optimum tree $T$}



==> _removed.tex <==
{\color{gray}

We provide a proof of the greedy algorithm. Assuming that there is an arbitrary allocation scheme initially, if there exists $b_i > b_j$, $f_{u} > f_v$ and $x_{uj},x_{vi}>0$, we can use the following transformation:
 
$$x_{uj} = x_{uj} - 1$$
$$x_{vi} = x_{vi} - 1$$
$$x_{ui} = x_{ui} + 1$$
$$x_{vj} = x_{vj} + 1$$
 
The difference of the objective function is:
$$\frac{f_u}{b_i}+\frac{f_v}{b_j}-\frac{f_{u}}{b_j} - \frac{f_v}{b_i} = (f_u-f_v)(\frac{1}{b_i} - \frac{1}{b_j}) < 0$$
 
This transformation can make the solution better, and we can use it until either $x_{uj}$ or $x_{vi}$ becomes $0$.

Therefore, in the optimal solution, if $b_i > b_j$, then 
$$\min_{x_{ui} > 0} f_u > \max_{x_{vj} > 0} f_v$$
 
This means that for a strictly decreasing $b$, the assigned $f$ must also be strictly decreasing, otherwise the above transformation can be used for improving the solution. For multiple identical $b$, the cost of assigning to any one of them is the same. Therefore, our greedy method can obtain an optimal solution to the LP.

Let $x$ be the solution obtained using this greedy algorithm; and $x$ is the optimum solution to the LP. Then, we can show the following inequality, which will lead to a $2$-approximation for this case.
\begin{align*}
    \sum_{i \in S, j \in T} \ceil{\frac{x_{ij}}{b_j}} \cdot f_i \leq 2 \cdot \sum_{i \in S, j \in T} \frac{x_{ij}}{b_j} \cdot f_i.
\end{align*}

For every $F \geq 0$, we define $S_F:= \{i \in S: f_i \geq F\}$.  To show the inequality, it suffices to show that for every threshold $F$, we have
\begin{align*}
    \sum_{i \in S_F, j \in T} \ceil{\frac{x_{ij}}{b_j}} \leq 2 \cdot \sum_{i \in S_F, j \in T} \frac{x_{ij}}{b_j}.
\end{align*}
Notice that $x_{ij} \in [0, b_j]$, and thus $\ceil{\frac{x_{ij}}{b_j}}$ is $0$ if $x_{ij} = 0$ and $1$ otherwise. Here is the informal argument for the above inequality. The difference between $\sum_{i \in S_F, j \in T} \ceil{\frac{x_{ij}}{b_j}}$ and $\sum_{i \in S_F, j \in T} \frac{x_{ij}}{b_j}$ is at most the number of sinks $t \in T$ that are ``split''.  This is at most the number of saturated sinks, which is at most $\sum_{i \in S_F, j \in T} \frac{x_{ij}}{b_j}$. }



%TODO: talk about why we only consider k = 3, 4, 5. Indeed, considering more values of k does not improve the approximation ratio. 

% \section{2-Approximation for fixed cost $f_{ij} = 1$ and arbitrary linear cost $c_{ij}$}

% {\color{gray}
% In this section, we consider the case where fixed cost $f_{ij} = 1$ but with the addition of arbitrary linear costs $c_{ij}$. We greedily minimizing the linear costs. This is a classical Minimum-cost Flow Problem, which can be transformed into a LP and solved in polynomial time complexity. We can perform flow adjustments by alternately coloring the cycles in black and white, ensuring that the selected edges form a forest structure without increasing the linear costs. This minimizes the number of edges selected in the solution, i.e. the fixed costs. The fixed cost of our method in the worst cases is $n+m-1$, while the optimal fixed cost not be less than $\max(n,m)$. And our method achieves the minimum linear cost, leading to a 2-Approximation.
% }

% {\color{gray} We consider a more special case PuFCT, where all $f_{ij}$ are same for $i \in S, j \in T$. We can assume all $f_{ij}=1$, and if all $f_{ij} = a$ ($a$ is a constant and greater than $0$), the optimum solution will be $a$ times when we set all $f_{ij}=1$. The problem is equivalent to selecting edges as few as possible to satisfy the requirement that the sources can be assigned to the sinks. 

% \subsection{Integer Programming}
% We can show that the edges we selected in the solution would not form any circle. This can be proved: when we find a circle consisted by the selected edges and a feasible assignment in currently solution, we alternately dye the edges of the circle in two colors, then choose the edge contained minimal units in the circle (suppose the minimum is $w$), decrease $w$ units from edges in same color as this edge and increase $w$ units to edges in different color. After the reassignment, the edge contained minimal units in the circle is unnecessary, leading to a better solution.

% If the problem contains $n$ sources and $m$ sinks, we just need to choose $(n+m-1)$ edges in the worst case, which would result in a spanning tree structure of the complete bipartite graph. Further edges chosen would form cycles, which are unnecessary. In fact, this number of edges is sufficient to satisfy the assignment requirements. We can eliminate cycles from any feasible solution or use same greedy strategy in PUFCT to obtain a solution with no more than $n+m-1$ edges chosen.

% Now, the question arises: can this solution be further improved? If we want to remove edges from the tree structure, the tree structure will split into multiple disconnected components. Since these components are disconnected, each of them needs to satisfy the supply and demand balance separately.

% Specifically, if we can partition $S\cup T$ into $k$ non-empty sets $V_1, V_2, ..., V_k$, such that each element from $S$ and $T$ belongs to exactly one of these sets, and for each set $V_d$, has $\sum_{i\in V_d \cap S} a_i = \sum_{j\in V_d \cap T} b_j$. Then we can split the tree into these $k$ disconnected components and require us to use only $n+m-k$ edges. The goal is to minimize $n + m - k$, or equivalently, to maximize $k$. The approximation ratio is defined using the minimization version.

% For all $V \subseteq S \cup T$ with $|V|\leq c$ and $\sum_{i\in V \cap S} a_i = \sum_{j\in V \cap T} b_j$, and some constants $c$ to be decided later, we have a variable $x_V \in \{0, 1\}$ indicating if $V$ is a set in the solution. Then, we consider the following integer programming:
% }


% \begin{equation*}
%     \min \qquad m + n - \sum_{V} x_V
% \end{equation*} \vspace*{-10pt}
% \begin{align*}
%     \sum_{V \ni v} x_V &\leq 1 &\quad &\forall v \in S \cup T\\
%     x_V &\geq 0&\quad &\forall V \subseteq S \cup T, 1\leq |V|\leq c
% \end{align*}

% {\color{gray}
% The constant $c$ restricts the maximum size of the sets $V$ we consider, i.e., sets of size less than or equal to $c$ must be determined whether they are in the solution. For a specific instance of the problem, if $c \geq n+m$, then the integer programming can obtain an exact solution to the problem; otherwise, it can provide an approximate solution. For a fixed constant c, finding all such sets $V$ is in polynomial time complexity.

% \subsection{$\frac{3}{2}$-Approximation where $c=2$}
% In this case, we only consider sets $\{i,j\}$ where $i \in S, j \in T$ and $a_i = b_j$. We try to find as many non-intersecting sets as possible. Since these sets have the constraint $a_i = b_j$, we simply need to find any such set $\{i,j\}$, remove $i$ and $j$ from $S$ and $T$ respectively, until no such set exists. We can prove that it does not make the solution worse. Suppose $a_i = b_j = t$. If a solution does not include set $\{i,j\}$, then there exists a node set $A \subseteq S$ where nodes in $A$ connect to $j$ and the sum of assigned values on the edges is $t$. Similarly, there exists a node set $B \subseteq T$ where $i$ connects to nodes in $B$, and the sum of assigned values is $t$. Let $|A| = x$ and $|B| = y$. Then, we can choose to remove these $x+y$ edges and choose the edge from $i$ to $j$. We can accomplish the assignment from node set $A$ to $B$ using no more than $x+y-1$ edges.

% Assuming we have found $x_2$ sets, we can obtain a predicted solution of $n+m-x_2-1$. Furthermore, one optimal solution can contain these $x_2$ sets and this optimal solution can include a maximum of $(n+m-2x_2)/3$ additional sets in the worst case because the size of the unconsidered sets are at least $3$. Therefore, the optimal solution will not be less than $n+m-x_2-(n+m-2x_2)/3-1 = \frac{2}{3}(n+m)-\frac{1}{3}x_2 - 1$, which will lead to a $\frac{3}{2}$-approximation for this case.

% \subsection{$c\geq 3$}

% It can be observed that the aforementioned integer programming is a classic set packing problem. Compared to the set packing problem, our problem is more special because our set $V$ is not arbitrary (must satisfy the supply and demand balance). The constant $c$ is equivalent to the bound size of the sets, converting the integer programming into a k-set packing problem. According to existing work, when $k \geq 3$, k-set packing is NP-hard, and Martin Furer and Huiwen Yu used a local improvement algorithm by Cygan to obtain an approximation ratio of $\frac{k+1}{3}+\epsilon$ for any $\epsilon>0$.

% We try to use this method to improve the approximation ratio of our method. We first eliminate all sets of size $2$, and the correctness of this step has been proven above. We define some variables: $x_i$ $(i \geq 3)$ to represent the selection of $x_i$ sets $V$ of size $i$ in the optimal solution, $z$ represent the total number of nodes (i.e., $n + m$), $opt$ represent the optimal solution and $sol$ represent the approximate solution of our method. Then, we scale these variables, where the optimal solution $opt$ is scaled to $1$, and the remaining variables are divided by $opt$. Specifically, the approximate solution $sol$ divided by $opt$ become the approximate ratio.
% For the case of $c = k$, we have following linear programming: }

% \begin{equation*}  
% \begin{aligned}  
%     & \max \ \ \   ratio \\
%     \pmb{s.t.}\ \  & z - \sum_{i=3}^{k+1} x_i = 1  && (1) \\  
%     & \sum_{i=3}^{k+1} i \cdot x_i = z && (2) \\  
%     & ratio \leq z - \frac{3}{4} x_3 && (3) \\  
%     & ratio \leq z - \frac{3}{5} (x_3 + x_4) && (4)\\  
%     & \vdots \\  
%     & ratio \leq z - \frac{3}{k+1} \sum_{i=3}^{k} x_i && (k)\\  
%     & x_i \geq 0, \forall i \in \{3, 4, \ldots, k+1\} \\  
%     & z,ratio \geq 0  
% \end{aligned}  
% \end{equation*}


% {\color{gray}
% This linear programming is equivalent to finding a worst case for our method. 
% Obviously, the worst case is when the sizes of the sets that are not considered in optimum solution are exactly $k+1$. Therefore, we introduce $x_{k+1}$ to represent these sets. The first constraint is that the optimal solution is equal to the total number of nodes minus the number of chosen sets; the second constraint is that the sum of the number of elements in chosen sets is equal to the total number of nodes. The following inequality represents that for any set size bound $j$ with $j \leq k$, we will use the corresponding k-set packing method for approximation, so we can obtain an approximate solution that contains at least $\frac{3}{j+1}$ sets. Here we temporarily ignore $\epsilon$ in the k-set packing approximation algorithm ratio.

% After testing different values of $c$, we found that the optimal approximation ratio of $\frac{6}{5}$ is achieved when $c=5$, and increasing the value of $c$ does not improve the approximation ratio. For $c=5$, the linear programming is as follows:
% }
    
% \begin{equation*}  
% \begin{aligned}  
%     & \max \ \ \   ratio \\
%     \pmb{s.t.}\ \  & z - x_3 - x_4 - x_5 - x_6 = 1 \\  
%     & 3x_3 + 4x_4 + 5x_5 + 6x_6 = z \\  
%     & ratio \leq z - \frac{3}{4} x_3 \\  
%     & ratio \leq z - \frac{3}{5} (x_3 + x_4) \\ 
%     & ratio \leq z - \frac{3}{6} (x_3 + x_4 + x_5) \\  
%     & x_3, x_4, x_5, x_6 \geq 0 \\  
%     & z,ratio \geq 0  
% \end{aligned}  
% \end{equation*}

% {\color{gray}
% This is a well-defined linear programming problem. By solving this linear programming, we obtain an optimal solution of $\frac{6}{5}$, which is achieved when $x_3:x_4:x_5 = 4:1:1$. Specifically, if $x_4 = x_5 = a$ and $x_3 = 4a$ (Note that since all variables need to be non-negative, the value of $a$ here is not arbitrary), we can solve for $z = \frac{6}{5} + 3a$, and the ratio is calculated as $ratio = z - \frac{3}{4} * 4a = z - \frac{3}{5} * 5a = z - \frac{3}{6} * 6a = \frac{6}{5}$. At this point, all the inequalities related to the ratio have reached their upper bounds.

% Next, we will prove that increasing the size of $c$ does not improve the result. We define the linear programming problem with $c=k$ as $LP_k$. Clearly, $opt(LP_k) \leq opt(LP_{k-1})$. This is because $LP_k$ considers a more set packing with size upper bound of $k$ in addition to $LP_{k-1}$, thus the constraints of the linear programming problem become stronger, which will result in a smaller optimal solution for maximization. 

% In addition, if $(x_3,...,x_{k-1}, x_k=0, ratio, z)$ is an optimal solution for $LP_{k-1}$, we can construct $(x_3,...,x_{k-1},x_k=0,x_{k+1}=0, ratio, z)$ as a feasible solution for $LP_k$. Since $x_k=0$, constraint $(k)$ in linear programming is weaker than constraint $(k-1)$, and it will not cause the value of $ratio$ to decrease. Then $opt(LP_{k}) \geq opt(LP_{k-1})$. When $c=5$, such an optimal solution appears for the first time. Specifically, the solution is $$(x_3=\frac{4}{15}, x_4=\frac{1}{15}, x_5=\frac{1}{15}, x_6=0, ratio=\frac{6}{5}, z=\frac{7}{5})$$.

% Therefore, we have shown that for $k \geq 6$, $opt(LP_{k}) = opt(LP_{k-1})$, and for $k \leq 5$, $opt(LP_k) \leq opt(LP_{k-1})$. So the best approximation ratio is achieved when $k=5$. Considering $\epsilon$ in the k-set packing algorithm approximation ratio, we obtain a $(\frac{6}{5} + \epsilon)$- approximate algorithm.

% We verify our conclusion when $c=5$ from the dual of the problem. Specifically, when $c=5$, the optimal solution is at least
% $$n+m-(x_3+x_4+x_5)-\frac{1}{6}(n+m-3x_3-4x_4-5x_5)=\frac{5}{6}(n+m)-\frac{1}{2}x_3-\frac{1}{3}x_4-\frac{1}{6}x_5$$
% Because the coefficient of $n+m$ is $\frac{5}{6}$, the approximation ratio will not be less than $\frac{6}{5}$, which corresponds to the case where only sets with sizes greater than 5 exist.

% For convenience, we multiply the optimal solution by $\frac{6}{5}$ to get
% $$n+m-\frac{3}{5}x_3-\frac{2}{5}x_4-\frac{1}{5}x_5$$

% Now, if we perform packing for sizes $\leq 4$, the approximate solution is
% $$n+m-\frac{3}{5}(x_3+x_4)$$

% It can be observed that when $0\leq x_5 \leq x_4$,
% $$\frac{3}{5}(x_3+x_4) \geq \frac{3}{5}x_3+\frac{2}{5}x_4+\frac{1}{5}x_5$$

% In this case, the approximation ratio reaches $\frac{6}{5}$.

% Otherwise, we set $x_4 = ax_5$ where $0 \leq a \leq 1$.
% If we perform packing for sizes $\leq 5$, the approximate solution is
% $$n+m - \frac{1}{2}(x_3+x_4+x_5)$$
% Let

% \begin{equation} 
% \frac{1}{2}(x_3+ax_5+x_5) \geq \frac{3}{5}x_3+\frac{2}{5}ax_5+\frac{1}{5}x_5 \label{c2}
% \end{equation}
% We get $x_3\leq (a+3) x_5$.

% If we perform packing for sizes $\leq 3$, the approximate solution is
% $$n+m - \frac{3}{4}x_3$$
% Let
% \begin{equation}
% \frac{3}{4}x_3 \geq \frac{3}{5}x_3+\frac{2}{5}ax_5+\frac{1}{5}x_5 \label{c3}
% \end{equation}
% We get $x_3 \geq (\frac{8}{3}a+\frac{4}{3})x_5$.

% When $0 \leq a \leq 1$, $a+3 \geq \frac{8}{3}a+\frac{4}{3}$. This means that for any $r=\frac{x_3}{x_5}$ at least one of the inequalities \eqref{c2} and \eqref{c3} will be satisfied. Specifically, when $a=1$, $a+3=\frac{8}{3}a+\frac{4}{3}=4$, which means that when $x_3:x_4:x_5=4:1:1$, the three approximate algorithms get the same approximation ratio of $\frac{6}{5}$. Considering $\epsilon$ in the k-set packing algorithm approximation ratio, we also get $(\frac{6}{5} + \epsilon)$-approximation ratio in the dual problem.
% }



{\medskip
\color{blue} (2024/11/5 written by Shi). $S_1, S_2, \cdots, S_k$ form a partition of $[m]$. $M$ is the set of $m' = \frac{m}{\epsilon}$ sinks incident to the $m'$ most expensive edges. That is, $M = S_1 \cup S_2 \cup \cdots \cup S_{t-1} \cup P_t$ for some $t$ and non-empty set $P_t \subseteq S_t$. 

We only need to focus on $M \triangle [m'] = ([m'] \setminus M) \cup (M \setminus [m'])$.

\begin{algorithm}[H] \color{blue}
    \begin{algorithmic}[1]
        \For{every $i \in [k]$}
            \State let $a'_i \gets b(S_i \cap (M \triangle [m']))$, $S'_i \gets S_i \setminus (M \triangle [m'])$
        \EndFor
        \State let $b'_j \gets b_j$ for every $j \in M \triangle [m']$
        \State $i \gets 1, j \gets $ first sink in $M \triangle [m']$
        \For{$i \gets 1$ to $k$}
            \While{$a'_i > 0$}
                \State $S'_i \gets S'_i \cup \{j\}, c \gets \min \{a'_i, b'_j\}, a'_i \gets a'_i - c, b'_j \gets b'_j - c$
                \State $j \gets $ the sink in $M \triangle [m']$ after $j$
                \If {$j$ does not exist} break the while loop and for loop \EndIf
            \EndWhile
        \EndFor
        \State $i \gets $ first source in $[k]$ with positive $a'$-value, $j \gets $ first sink in $M \triangle [m']$ with positive $b'$-value
        \While{$i \leq k$}
            \State $S'_i \gets S'_i \cup \{j\}, c \gets \min\{a'_i, b'_j\}, a'_i \gets a'_i - c, b'_j \gets b'_j - c$
            \If{$a'_i = 0$} $i \gets i + 1$ \EndIf
            \If{$b'_j = 0$} $j \gets $ first sink in $M \triangle [m']$ with positive $b'$-value \EndIf
        \EndWhile
    \end{algorithmic}
\end{algorithm}
}

{\medskip
\color{gray} (2024/10/22 written by Shi). This section is on how we convert an optimum solution to a $(1+\epsilon)$-approximately optimum solution with the property that the first few expensive edges are incident to the sinks with the largest demands.

\paragraph{The setting} We are given $m$ sinks indexed as $[m]$, and the demands are $b_1 \geq b_2 \geq \cdots \geq b_m$. There are $k$ sources denoted as $[k]$, where $k$ is a parameter in for our FPT algorithm. We have fixed costs for the sources, satisfying $f_1 \geq f_2 \geq \cdots \geq f_k$. Each source $i \in [k]$ has $a_i$ units of supply, and $a([k]) = b([m])$.  Let $m' = \frac{k}{\epsilon}$ for some small enough $\epsilon > 0$. We assume $m'$ is an integer. 

We are given a solution $\OPT$ to the problem where every sink is connected to exactly one source. So, let $S_i$ for every $i \in [k]$ be the set of sinks connected $i$ in $\OPT$.  So $(S_i)_{i \in [k]}$ form a partition of $m$ and $b(S_i) = a_i$ for every $i \in [k]$. Moreover, we assume there is a $t \in [k]$ such that $\sum_{i \in [t]}|S_i| = m'$. Most of the time in this section, we only focus on the sets $S_1,  S_2, \cdots, S_t$.

The main theorem we prove is
\begin{theorem}
    TODO: need to think about the exact statement for the theorem. 
\end{theorem}


Let $T = \big(\union_{i \in [t]} S_i\big) \cap [m']$.

Consider the following procedure for constructing two families of sets $S'_1, S'_2, \cdots, S'_t$, and $S''_1, S''_2, \cdots, S''_t$.
\begin{algorithm}[H]
    \color{gray}
    \begin{algorithmic}[1]
        \For{every $i \in [t]$}: let $S'_i \gets S_i \cap [m'] = S_i \cap T$ \EndFor
        \State $T' \gets [m'] \setminus T$
        \For{every $i \in [t]$} 
            \While{$b(S'_i) < a_i$}
                \State $j \gets$ smallest-index sink in $T'$
                \State $S'_i \gets S'_i \cup \{j\}$
                \State $T' \gets T' \setminus \{j\}$
            \EndWhile
        \EndFor
    \end{algorithmic}
\end{algorithm}

The procedure is well-defined. The sets $S'_i, i \in [t]$ are disjoint subsets of $[m']$.

All the sinks in $S'_i \setminus S_i$ are in $[m'] \setminus T$, and all the sinks in $S_i \setminus S'_i$ are outside $[m']$.

Let $d_i := |S_i| - |S'_i| \geq 0$ for every $i \in [t]$, and let $d = \sum_{i \in [t]} d_i$. Let $R = [m] \setminus \union_{i \in [t]} S_i$. 

For each $i \in [t]$, we match the $a_i$ units of the supply at source $i$ with the $b(S'_i) \geq a_i$ units of demands in $S'_i$, with following two conditions satisfied:
\begin{itemize}
    \item For every sink $j \in S_i \cap S'_i$, the $b_j$ units of demand at $j$ is fully matched. 
    \item In case of $b(S'_i) > a_i$, the unmatched demand is on a single sink $j$, which is in $S'_i \setminus S_i$. 
\end{itemize}
The two properties can be satisfied. Then, for every $j \in [m]$, we let $b'_j$ be the amount of unmatched demands at sink $j$. In particular, for every $j \notin \union_{i \in [t]} S'_i$, we have $b'_j = b_j$. For every $i \in [t]$, we have at most one sink $j \in S'_i$ with $b'_j > 0$, and it must be in $S'_i \setminus S_i$, if it exists.  This means that sinks $j \in T$ have $b'_i = 0$.

\begin{lemma}
    For every $i \in [t]$ and positive integer $p \leq |S'_i \setminus S_i|$, the following condition holds: the sum of the $p$ largest values in $\{b_j: j \in S'_i \setminus S_i\}$ is at most the sum of the $p + d_i + 1$ largest values in $\{b'_j: j \in S_i \triangle S'_i\}$.
\end{lemma}
\begin{proof}
    
\end{proof}

\begin{lemma}
    For every integer $p \in [|R|]$, the sum of the $p$ largest values in $\{b_j: j \in R\}$ is at most the sum of the $p + d + k$ largest values in $\{b'_j: j \in [m]\}$.
\end{lemma}
\begin{proof}
    This follows from the previous lemma. 
\end{proof}

}


\remove{
\begin{theorem}  
    {\color{red} Summary the conclusions that be proof in Section 3}
\end{theorem}

\begin{theorem} 
    In the PFCT-S problem, since $\forall j,k\in T, f_{ij}=f_{ik}$, we can use $f_{i}$ represent $f_{ij}$. We first sort $S$ in descending order by $f_{i}$ and sort $T$ in descending order by $b_i$. We transport the products of sources in $S$ in foregoing order. The sinks in $T$ also receive commodities from sources in order. So when the current sink's demand has been met, we will let the next sink to accept commodities until all commodities are transported. We can show that this method can achieve our goal with a cost no more than twice of the optimal solution(i.e. a 2-approximation algorithm). This theorem is proved through relaxation of the integer programming form of FCT problem.
\end{theorem}

\begin{theorem}  
    We define that if a set $V$ satisfies $\sum_{i\in V \cap S}a_i = \sum_{i\in V \cap T}b_j$, then $V$ is a balanced subset. It can be proved that maximizing the number of disjoint balanced subsets is equivalent to solving the PFCT-U problem. Therefore, we reduce the PFCT-U problem to a $k$-set packing problem. According to the algorithm in \cite{FY}, we can obtain an $\frac{k+1+\epsilon}{3}$ approximate solution of $k$-set packing problem. We finally obtain an approximate solution of $6/5 + \epsilon$ for PFCT-U problem. We also show that only need to consider the balanced subsets $V$ have $|V|\in \{3,4,5\}$ can obtain this approximation ratio. In other words, considering larger balanced subsets would not result in a better approximation ratio. Additionally, we can show this approximation ratio is tight.    
\end{theorem}

\begin{table}[h] %voc table result 
    \color{gray}
    \caption{Brief results of FCT problem and relevant special cases}
    \label{Results}
    \renewcommand{\arraystretch}{2}
    \centering
        \begin{tabular}{*{4}{c}}
            \toprule
            Case Name & Results\\
            \midrule
            FCT & {\color{red} results of FCT} \\
            PFCT & {\color{red} results of PFCT} \\
            FCT-S & {\color{red} results of FCT-S} \\
            PFCT-S & $2$-approximation greedy algorithm \\
            FCT-U & $2$-approximation Minimum-cost Flow algorithm \\
            PFCT-U & $(\frac{6}{5}+\epsilon)$-approximation k-sat packing algorithm \\
            \bottomrule
        \end{tabular}
\end{table}
}

\remove{
\paragraph{Densest-$k$-Subgraph Problem and its Dual} In the Densest-$k$-Subgraph (DkS) problem, we are given a graph $G = (V, E)$ and an integer $k > 0$, and the goal of the problem is to find a set $S \subseteq V$ of $k$ vertices, so as to maximize the number of edges in $G[S]$, the subgraph of $G$ induced by $S$.  A closely related problem is the Dual Densest-$k$-Subgraph (Dual-DkS) problem. Given a graph $G = (V, E)$, and an integer $\ell > 0$. The goal is to find a smallest set $S \subseteq V$ such that the number of edges in $G[S]$ is at least $\ell$.

The DkS problem was introduced by Kortsarz and Peleg \cite{KP}, who provided an $O(n^{2/5})$ ratio for the problem. The current best-known approximation ratio for DkS, due to Bhaskara et al. \cite{BCC},  is $O(n^{1/4+\epsilon})$ for any arbitrarily small constant $\epsilon>0$.  For the Dual-DkS problem, t he best known approximation ratio is $O(n^{3-2\sqrt{2}+\epsilon})$, for arbitrarily small constant $\epsilon>0$ \cite{CDK}. 

On the hardness side, a breakthrough result due to Manurangsi \cite{M17} demonstrated that, under the Exponential Time Hypothesis (ETH), there is no $n^{(\log\log n)^c}$-approximation for DkS. Under a stronger complexity assumption known as the Gap-ETH assumption, he further showed that there is no $n^{f(n)}$-approximation for any function $f(n) \in o(1)$. More recently, Chuzhoy et al.\cite{CDG} proved that DkS cannot be approximated within a factor of $2^{\log^{\epsilon}n}$ for some constant $\epsilon>0$, assuming a novel conjecture they introduced on the hardness of some constraint satisfaction problems. A simple reduction shows that the approximation ratios of the two problems are polynomially related, implying that all the hardness results mentioned above also apply to the Dual-DkS problem.}


% Whenever only ﬁxed costs are considered and all variable costs are zero, the FCT problem becomes the pure ﬁxed charge transportation (PFCT) problem\cite{FM, GL}. Obviously, the PFCT problem is a special case of FCT. It corresponds to a specific scenario in transportation problems under the condition that the costs of goods transportation is much lower than the costs of route establishment, such as pipeline systems and electric power systems. To solve PFCT problem, \cite{FM} proposed a search method to get exact solution using some decision rules, while \cite{GL} reformulated the PFCT problem as an equivalent set covering problem and used heuristics combined with constraints generated from maximum flow problems.

% Although the FCT problem and PFCT problem have attracted considerable research attention in the literature, such as exact solution methods\cite{M,G,AA,ZLRP,MR}, branch-and-bound algorithms\cite{KU,BGK,CE,RBM} and heuristic algorithms\cite{WH,SAMD,GAK,A09,EA,LT,BRT}, to the best of our knowledge, its complexity and approximation algorithms have not been studied in great detail in the past. The only known results show that the FCT problem is NP-hard\cite{GP} and the PFCT problem is also NP-hard\cite{K05,SFC}. 

% \begin{table}[] 
% \centering  
% \caption{Notation Table of our paper}  
% \label{tab:notation}  
% \begin{tabular}{cl}
% \midrule
% $S$ & Source nodes set \\ 
% $T$ & Sink nodes set \\
% $n = |S|$ & source nodes size\\
% $m = |T|$ & The number of source nodes \\
% $a_i$ & Commodities units in the $i$-th source \\  
% $b_i$ & Commodities units in the $i$-th sink \\
% edge $(i,j)$ & Route from $i$-th source to $j$-th sink \\
% $c_{ij}$ & Variable (linear) cost of edge $(i,j)$ \\
% $f_{ij}$ & Fixed cost of edge $(i,j)$ \\
% $x_{ij}$ & Commodities units transported along edge $(i,j)$ in a scheme\\ 
% \bottomrule 
% \end{tabular}  
% \end{table}  


% Note: the introduction before modified is follow.

% In 1954, Hirsch and Dantzig ﬁrst introduced the ﬁxed charge transportation (FCT) problem where the cost for sending goods from a source to a sink is equal to a variable cost proportional to the amount of goods sent plus a ﬁxed cost\cite{HD54, HD68}. The FCT problem generalizes the well-known classical transportation problem in the sense that additional to variable transportation costs the forwarders are charged with ﬁxed costs for establishing a route. 

% The FCT problem is a special case of the single commodity uncapacitated ﬁxed-charge network problem\cite{RW, OW}, which is a special case of a large class of network design problems\cite{A, FG, RKOW}.

% The FCT problem is a general model for several practical problems in distribution, transportation, scheduling, and location systems, where the ﬁxed costs may represent toll charges on highways, landing fees at airports, setup costs in production systems, or costs for building roads. Real-life applications of the FCT problem are also described in \cite{S, W, JURM, PKZ, HC, AK}.

% Whenever only ﬁxed costs are considered and all variable costs are zero, the FCT problem becomes the pure ﬁxed charge transportation (PFCT) problem\cite{FM, GL}. 

% Although the FCT prolbem and PFCT problem have attracted considerable research attention in the literature, such as exact solution methods\cite{M,G,AA,ZLRP,MR}, branch-and-bound algorithms\cite{KU,BGK,CE,RBM} and heuristic algorithms\cite{WH,SAMD,GAK,A09,EA,LT,BRT}, to the best of our knowledge, its complexity and approximation algorithms have not been studied in great detail in the past. The only known results show that the FCT problem is NP-hard\cite{GP} and the PFCT problem is also NP-hard\cite{K05,SFC}. 

% Although the FCT problem has been extensively studied and yet is still poorly understood for its computational complexity and approximation algorithm. In this paper, we first give a comprehensive complexity analysis for the FCT problem and PFCT problem, which greatly complements the research gap of this problem. Then, we design efficient approximation algorithms to deal with each NP-hard cases.  


% In the \emph{Fixed Charge Transportation (FCT) problem}, we are given a set $S$ of sources and a set $T$ of sinks. Each $i \in S$ has a $a_i \in \Z_{>0}$ units of supply and each $j \in T$ has $b_j \in \Z_{>0}$ units of demand.  We have $\sum_{i \in S} a_i = \sum_{j \in T}b_j$. We are given a variable cost of transporting one unit of the
% commodity from source node $i$ to sink node $j$ is $c_{ij} \in \R_{\geq 0}$ and a fixed cost $f_{ij} \in \R_{\geq 0}$ whenever transporting occurs from source node $i$ to sink node $j$ for every $i \in S, j \in T$. 

% In the output of the problem, we specify non-negative values $x_{ij}$ representing the amount of commodity transported along the edge  $(i,j)$. Therefore, the following equalities need to be satisfied: $\sum_{j \in T}x_{ij} = a_i, \forall i \in S$ and $\sum_{i \in S}x_{ij} = b_j, \forall j \in T$.  Our goal is to minimize the cost of the solution $x$, which is defined as 
% \begin{align*}
%     \sum_{i \in S, j \in T}\left(1_{x_{ij}>0}\cdot f_{ij} + x_{ij}\cdot c_{ij}\right). 
% \end{align*}


% %and binary variables $y_{ij}$ taking a value $1$ if and only if $x_{ij}$ is positive  (i.e., edge $(i,j)$ is used). Let $d_{ij}=min \{a_i, b_j\}$. The FCTP can be formulated as follows. 
% % \begin{equation}
% %     \min \sum_{i \in S, j \in T} x_{ij}\cdot c_{ij}+ y_{ij}\cdot f_{ij} \label{LP1}
% % \end{equation}
% % \begin{align*}
% %     \sum_{j \in T}x_{ij} &= a_i &\quad &\forall i \in S\\
% %     \sum_{i \in S}x_{ij} &= b_j &\quad &\forall j \in T\\
% %     x_{ij} &\leq d_{ij}\cdot y_{ij} &\quad &\forall i \in S, j \in T\\
% %     x_{ij} &\geq 0 &\quad &\forall i \in S, j \in T\\
% %     y_{ij} &\in \{0, 1\}&\quad &\forall i \in S, j \in T
% % \end{align*}

% Therefore, there are 6 special cases of the FCT problem, depending on whether we have the linear costs $c_{ij}$'s, and how special the fixed costs $f_{ij}$'s are. The 6 special cases are defined as FCT, FCT-S, FCT-U, PFCT, PFCT-S, PFCT-U respectively. 


% % In the Pure Fixed Charge Transportation (PFCT) problem, we are given a set $S$ of sources and a set $T$ of sinks. Each $i \in S$ has a $a_i \in \Z_{>0}$ units of supply and each $j \in T$ has $b_j \in \Z_{>0}$ units of demand.  We have $\sum_{i \in S} a_i = \sum_{j \in T}b_j$. We are given a cost $f_{ij} \in \R_{\geq 0}$ for every $i \in S, j \in T$. The goal of the problem is to find a vector $x \in \R_{\geq 0}^{S \times T}$ such that 
% % \begin{align*}
% %     \sum_{j \in T} x_{ij} &= a_i &\quad &\forall i \in S,\\
% %     \sum_{i \in S} x_{ij} &= b_j &\quad &\forall j \in T,
% % \end{align*}
% % so as to minimize $\sum_{i \in S, j \in T}1_{x_{ij} > 0} \cdot f_{ij}$.

% % A special case of PFCT problem is when the costs $f_{ij}$ only depend on the source $i$. That is, there is a $f_i \in \Z_{\geq 0}$, such that $f_{ij} = f_i$ for every $i, j$. We use PFCT-S to denote the special case. 
%only fixed costs are considered; only fixed costs are considered and the fixed costs are equal for the same source; the fixed costs are equal for all edges( edges can be considered as 1 without loss of generality); only fixed costs are considered and the fixed costs are equal for all edges. The name of these cases, additional conditions (compared to the original FCT problem), and the objective functions are summarized in the table \ref{Specialcase}.

% \begin{table}[h] %voc table result
%     \caption{Relevant special cases of FCT}
%     \label{Specialcase}
%     \renewcommand{\arraystretch}{2}
%     \centering
%         \begin{tabular}{*{4}{c}}
%             \toprule
%             Case Name & Additional Constraints & Objective Function\\
%             \midrule
%             PFCT & $c_{ij}=0$ & $\min_{x} \sum_{i \in S, j \in T}\left(1_{x_{ij}>0}\cdot f_{ij} \right)$ \\
%             PFCT-S & $c_{ij}=0$, $\forall j,k \in T, f_{ij} = f_{ik}$ & $\min_{x} \sum_{i \in S, j \in T}\left(1_{x_{ij}>0}\cdot f_{ij} \right)$ \\
%             % FCT-U & $f_{ij}=1$ & $\min_{x} \sum_{i \in S, j \in T}\left(1_{x_{ij}>0} + x_{ij}\cdot c_{ij}\right)$ \\
%             PFCT-U & $c_{ij}=0$, $f_{ij}=1$ & $\min_{x} \sum_{i \in S, j \in T}\left(1_{x_{ij}>0}\right)$ \\
%             \bottomrule
%         \end{tabular}
% \end{table}

%We also consider many special cases of the FCT problem, depending on the fixed costs and linear costs. 



%first give a comprehensive complexity analysis for the FCT problem and PFCT problem, which greatly complements the research gap of this problem. Then, we design efficient approximation algorithms to deal with each NP-hard cases. After researching these cases, we have reached the following main conclusions. (Table \ref{Results} give a brief overview about our conclusions in each cases.)
%
%
%Our first theorem shows the other reduction:
% Shi: I think there is no need to formally state the theorem. 
% \begin{theorem}
%     Given a FCT-Digraph (PFCT-Digraph) instance, we can efficient construct a FCT (PFCT) instance, such that 
%     \begin{itemize}
%         \item There is a one-to-one correspondence between the valid solutions for the FCT-Digraph (PFCT-Digraph) instance and the valid solutions for the FCT (PFCT) instance. Two correspondent solutions have the same cost to their respective problems. 
%         \item Given 
%     \end{itemize}
% \end{theorem}

% Our first result is a pseudo-quasi-polynomial time algorithm for the FCT-Digraph problem:
% \begin{theorem}
%     There is an $n^{O(\log n \cdot \log (nf_{\max}))}$-time $O(\log^2n)$-approximation algorithm for the FCT-Digraph problem, where $f_{\max} := \max_{e \in E} f_e$ is the maximum fixed cost over all edges.
% \end{theorem}
% \begin{theorem}  
%     In the FCT-U problem, we first ignore the fixed costs $f_{ij}$ and solve for the minimum cost flow with variable cost $c_{ij}$. Then we pay the fixed costs for the edges with flow and calculate the total costs. We can prove that this scheme can achieve the minimum variable cost, and the fixed costs do not exceed twice the optimal fixed costs when $f_{ij} = 1$, which results in a 2-approximate algorithm. 
    
% \end{theorem}



    % NO NEED TO GROUP
    % The support of $y_{ij}$ is a forest. Wlog, we assume it is a tree $\bfT$; if this is not the case, we can consider each tree separately. We shall get a new solution $y'$ as follows. We root $\bfT$ at an arbitrary vertex $r \in S \cup T$. For every vertex $v \in S \cup T$, we group the child-edges of $v$ according to their $C$-values. For every group $E'$ of edges with the $C_{ij}$ values being $C$, we construct a vector $y' \in [0, 1]^{E'}$ such that 
    % \begin{itemize}
    %     \item $y'_e = y_e$ if $y_e \geq \epsilon$,
    %     \item $y'_e \in \{0, \epsilon\}$ if $y_e < \epsilon$,
    %     \item $\sum_{e \in E'} y'_e - \sum_{e \in E'} y_e \in (-\epsilon, 0]$, and
    %     \item $\sum_{e \in E'} (f_e + \frac{c_e}{C}) y'_e \leq \sum_{e \in E'} f_e y_e$.
    % \end{itemize} 
    % That is, if $y_e \in [\epsilon, 1]$, we then keep it unchanged. Otherwise, $y_e \in [0, \epsilon)$ and we need to change it to either $0$ or $\epsilon$. We can do so without changing $\sum_{e \in E'}y_e$ and $\sum_{e \in E'}f_e y_e$ unchanged, until when there is at most one edge $e\in E'$ with $y_e \in (0, \epsilon)$. Then we simply change $y_e$ to $0$. So, the properties can be guaranteed.

    % Once we obtain the vector $y'$, we can define $x'_{ij} = C_{ij}y'_{ij}$ for every $i \in S, j \in T$.  We output $x'$ as our solution. For every $i \in S$, we have $\sum_{j \in T} C_{ij} y'_{ij} - \sum_{j \in T} C_{ij} y_{ij}  \leq 2\epsilon a_i$, where the difference can only come from the parent edge of $i$. On the other hand,
    % \begin{align*}
    %      \sum_{j \in T} C_{ij} y_{ij} - \sum_{j \in T} C_{ij} y'_{ij} \leq \epsilon\cdot 2a_i + \left(2a_i + a_i + \frac{a_i}{2} + \frac{a_i}{4} + \cdots \right) \cdot \epsilon \leq 6\epsilon a_i. 
    % \end{align*}
    % Above, the first $\epsilon \cdot 2a_i$ comes from the parent edge of $i$, and the second term comes from the groups of children edges of $i$. Therefore, for every $i \in S$, we have
    % \begin{align*}
    %     \sum_{j \in T} C_{ij} y'_{ij} - \sum_{j \in T} C_{ij} y_{ij}  \in [-6\epsilon a_i,2\epsilon a_i].
    % \end{align*}
    % Similarly, for every $j \in T$, we have 
    % \begin{align*}
    %     \sum_{i \in S} C_{ij} y'_{ij} - \sum_{i \in S} C_{ij} y_{ij}  \in [-6\epsilon b_j,2\epsilon b_j].
    % \end{align*}
    
    % Therefore, we have a flow $x' \in \R_{\geq 0}^{S \times T}$ where the amount of flow sent by each $i\in S$ is between $(1-6\epsilon)a_i$ and $(1+2\epsilon)a_i$, and the flow received by each $j \in T$ is between $(1-6\epsilon)b_j$ and $(1+2\epsilon)b_j$. We can scale the all $x'$ values within a factor between $\frac{1}{1+2\epsilon}$ and $\frac{1}{1-6\epsilon}$ so that 
    % \begin{itemize}
    %     \item every source $i$ sends exactly $a_i$ units flow
    %     \item every sink $j$ receives between $\frac{1-6\epsilon}{1+2\epsilon}\cdot b_j$ and $\frac{1+2\epsilon}{1-6\epsilon}\cdot b_j$ units of flow. 
    % \end{itemize}
    % We can scale down the $\epsilon$ value at the beginning so that in the end so that the flow received by each $j$ is within $(1\pm \epsilon)b_j$.  The cost of $x'$ to the FCT instance is 
